Two Models are Better than One: Federated Learning Is Not Private For Google GBoard Next Word Prediction

In this paper we present new attacks against federated learning when used to train natural language text models. We illustrate the effectiveness of the attacks against the next word prediction model used in Google's GBoard app, a widely used mobile keyboard app that has been an early adopter of federated learning for production use. We demonstrate that the words a user types on their mobile handset, e.g. when sending text messages, can be recovered with high accuracy under a wide range of conditions and that counter-measures such a use of mini-batches and adding local noise are ineffective. We also show that the word order (and so the actual sentences typed) can be reconstructed with high fidelity. This raises obvious privacy concerns, particularly since GBoard is in production use.

==> dlg.tex <==
In our attack context, DLG can recover words but at much smaller
scales and takes longer to find these words. There is also no
guarantee that DLG can recover words and place them in the correct
order. In \cite{zhu2019dlg}, it is noted that the algorithm requires
multiple restarts before successful reconstruction. Additionally, DLG
operates by matching the single gradient of a batch of training data,
therefore it only works in the FedSGD setting, where $E = 1$. We show
the results of DLG in Listing \ref{lst:sampledlg} on gradients of
$B = 1, \mbox{ and } 2$ 4 word sentences. In the first example, it
took DLG 1000 iterations to produce ``\texttt{<S> how are venue}'',
and 1500 iterations to produce ``\texttt{<S> how are sure cow},
\texttt{<S> haha where are Tell van}''. These reconstructions include
some of the original words, but recovery is not as precise as our
attack, and takes orders of magnitude longer to carry out.

\begin{lstlisting}[frame=single,caption=Original and reconstructed sentences by DLG,label=lst:sampledlg]
  <S> how are you
  <S> how are venue

  <S> how are you doing 
  <S> how are sure cow  
  <S> where are you going
  <S> haha where are Tell van
\end{lstlisting}

